CaLM: Contrasting Large and Small Language Models to Verify Grounded Generation

Grounded generation aims to equip language models (LMs) with the ability to produce more credible and accountable responses by accurately citing verifiable sources. However, existing methods, by either feeding LMs with raw or preprocessed materials, remain prone to errors. To address this, we introduce CaLM, a novel verification framework. CaLM leverages the insight that a robust grounded response should be consistent with information derived solely from its cited sources. Our framework empowers smaller LMs, which rely less on parametric memory and excel at processing relevant information given a query, to validate the output of larger LMs. Larger LM responses that closely align with the smaller LMs' output, which relies exclusively on cited documents, are verified. Responses showing discrepancies are iteratively refined through a feedback loop. Experiments on three open-domain question-answering datasets demonstrate significant performance gains of 1.5% to 7% absolute average without any required model fine-tuning.

==> 02-prelim.tex <==
\begin{figure*}[ht!]
\centering 
\includegraphics[width=0.99\textwidth]{Figures/prelim_fig.pdf} 
\vspace{-2pt}
\caption{
The studies of the performance of an LM as a function of the input document's relevance score using the ASQA dataset.
We show that, \textit{within the same LM family, smaller LMs demonstrate higher sensitivity to the relevance of the input document to query $q$, when anchored to the largest model in the family}.
\textbf{\textit{(a)}} The illustration of the function. This function is a monotonic increase function as the accuracy always increase when input document's relevance score increase. Hence, studying the second order relative improvements can help us know the \textit{incremental performance gain} for the LM when the input document's relevance to query $q$ keep increasing.
\textbf{\textit{(b)}} The result of relative improvement.
\textbf{\textit{(c)}} The result of our second order relative improvement analysis. 
From (b)(c), in contrast of larger model, we can observe that smaller models usually get higher relative improvements and larger incremental performance gain.
}
\vspace{-8pt}
\label{fig:prelim} 
\end{figure*}

\section{Background and Motivation}
\label{sec:preliminary}

\subsection{Problem Statement}
We cope with the task of grounded generation~\cite{gao-etal-2023-enabling}.
Given a query $q$ and a corpus of trustworthy text passages $\mathcal{D}$, the model needs to generate an answer $\mathcal{A}$, which consists of $n$ statements $s_1, s_2, ... s_n$, based on the knowledge in $\mathcal{D}$.
Each statement $s_i$ cites a list of passages $\mathcal{C}_i=\{c_i^1, c_i^2, ...\}, \forall c_i^j \in \mathcal{D}$. 
The collective sets $\mathcal{C}_i$ for $i=1,2,\ldots,n$ constitute the grounded evidence $\mathcal{G}$, from which $\mathcal{A}$ is derived.
Our goal is to jointly optimize the usefulness of $\mathcal{A}$ to $q$, the preciseness of $\mathcal{C}_i$ for statement $s_i$, and the integrity of $\mathcal{G}$ to adequately support $\mathcal{A}$.





\subsection{Verification of Grounded Generation}
\label{sec:motivation}
%Although LLMs have demonstrated proficiency in a wide range of tasks, a significant challenge they face is the tendency to generate hallucinations~\cite{DBLP:journals/corr/abs-2311-05232, DBLP:journals/corr/abs-2309-01219}.
%Given the high complexity of grounded generation task, such hallucinations in answers or citations are somewhat inevitable. This issue underscores the necessity of implementing verification mechanisms for the answers provided by LLMs to maintain the quality of the final output $\mathcal{A}$.

Although LLMs have demonstrated proficiency in a wide range of tasks, they remain susceptible to generating hallucinations~\cite{DBLP:journals/corr/abs-2311-05232, DBLP:journals/corr/abs-2309-01219}. These hallucinations persist in answers or citations within grounded generation tasks due to its complexity. This issue underscores the critical need for implementing verification mechanisms to ensure the quality of the final output $\mathcal{A}$.


The optimization goals for grounded generation are threefold: ensuring the correctness of the answer $\mathcal{A}$, maintaining the integrity of $\mathcal{G}$ to support $\mathcal{A}$, and ensuring high-quality citations for each statement. We aim to devise strategies to verify the first two objectives, while citation quality assessment can be accomplished through a trained Natural Language Inference (NLI) model~\cite{gao-etal-2023-enabling}. However, since evaluating citation quality with NLI models mirrors the final system evaluation process, we opt not to employ NLI models in our method to ensure a fair comparison.

Our design draws inspiration from exploiting the inherent characteristics of small LMs. 
We posit that a robust $\mathcal{G}$ should enable even small LMs to deduce the correct answer.
Notably, small LMs, having fewer parameters, are shown to be more open to integrate external knowledge~\cite{DBLP:journals/corr/abs-2305-13300}.\footnote{In this paper, we distinguish between LMs based on size, referring to them as large and small LMs. However, it is more accurate to categorize them as strong and weak LMs to reflect the varying levels of performance across different LM families.}
Furthermore, as we will detail in \Cref{sec:explore_LM}, smaller LMs exhibit greater sensitivity to the relevance of input documents to query $q$.
The presence of irrelevant documents in the evidence set $\mathcal{G}$ provided to small LMs can easily lead to erroneous results and suboptimal performance.
Driven by these insights, we propose employing smaller LMs as verifiers to assess the accuracy of answers $\mathcal{A}$ generated by the LLM, enhancing reliability and accuracy.




\subsection{Analyzing Model Size Impact on LMs' Sensitivity to Input Document Relevance}
\label{sec:explore_LM}
In this section, we aim to demonstrate that smaller LMs exhibit higher sensitivity to the relevance of the input document to query $q$ than the largest LMs of the same model family.

We investigate the sensitivity of LMs to the relevance of input documents through both relative performance gain analysis and second-order improvements gain analysis. 
As depicted in \Cref{fig:prelim}(a), the performance of an LM as a function of the input document's relevance typically exhibits a monotonic increase. 
To mitigate the effects of the models' divergent abilities to follow instructions, we first examine the relative performance improvement of the model response as the relevance of the input document increases. 
The larger this value is, the more sensitive the LM is.

Moreover, acknowledging the potential complexity of this function beyond simple linearity, we also conduct a second-order analysis. 
This analysis use three anchoring points $x_{low}, x_{med}, x_{high}$ and the corresponding performance $P(x_{low}), P(x_{med}), P(x_{high})$ to study the much incremental performance gain the LM can get when the input document's relevance keep increasing. Specifically, we use the ratio $\tfrac{P(x_{high})-P(x_{med})}{P(x_{med})-P(x_{low})}$ to represent the incremental performance gain.
A higher ratio indicates LM is more sensitive to input document's relevance, as illustrated by the orange line in \Cref{fig:prelim}(a).

\begin{figure*}[ht!]
\centering 
\includegraphics[width=0.95\textwidth]{Figures/Overview_v1.pdf} 
\vspace{-7pt}
\caption{Overview of \mymodel{}: \textit{\textbf{Top:}} The flow diagram of our method. \textit{\textbf{Bottom:}} A detailed depiction of each step's operation. The algorithm starts with a retriever extract a relevant document pool $p$ for the input query (Step (1)).
Then, the main language model (LM) takes the first batch of documents and employs retrieval-augmented generation to produce an answer candidate, which cites relevant supporting documents (Step (2)). 
Subsequently, this candidate is validated by contrasting it with the verifier output from the verifier LM (Steps (3) \& (4)). 
Our verifier LM evaluates citation quality by accessing only the documents cited by the main LM's response, rather than the same input documents. For responses with sufficient consistency, we accept the answer candidate directly. 
If inconsistent, we break down the answer candidate into individual statements, retaining only those corroborated by similar arguments in the verifier output for further correction in next iteration (Step (5)).}
% For generative QA tasks, the consistency measurement is done by calculate ROUGE-2 scores between the answer candidate and verifier output. 
% For extractive QA, exact string match is used.
% To prepare input for next iteration, an active document search process is adapted to increase the likelihood of finding relevant documents.}
\vspace{-8pt}
\label{fig:overview} 
\end{figure*}


We conduct empirical studies using a retrieval-augmented generation setting on the ASQA dataset~\cite{DBLP:conf/emnlp/StelmakhLDC22}. Each instance in the dataset contains multiple answers and requires reading multiple documents to make correct prediction. 
In this experiment, a LM utilizes five input documents $\mathbf{d}$ to answer queries $q$, with model performance evaluated based on answer accuracy, and the relevance of the input documents $\mathbf{d}$ is assessed by their average recall rate in containing answers.
We prepare three different set of $\mathbf{d}$ with approximately 27\%, 56\%, and 78\% recall rates, respectively, to represents $x_{low}, x_{med}, x_{high}$ in \Cref{fig:prelim}(a).
\Cref{fig:prelim}(b) presents the results of relative performance improvement, while \Cref{fig:prelim}(c) shows the second-order analysis. Our study encompasses LM families such as Yi-LM~\footnote{https://github.com/01-ai/Yi}, Vicuna~\cite{DBLP:journals/corr/abs-2306-05685}, WizardLM~\cite{DBLP:journals/corr/abs-2304-12244}, and Tulu-2-dpo~\cite{DBLP:journals/corr/abs-2311-10702}. 
The findings indicate that within the same LM family, compared to the largest model, smaller LMs usually achieve higher relative improvement and receive a greater incremental performance gain, suggesting their higher sensitivity to the relevance of input documents to the query $q$.
On the other hand, smaller LMs are more prone to erroneous results and suboptimal performance with irrelevant documents, which motivates our design choice of verification method.



